Transformer-based Planning for Symbolic Regression

Symbolic regression (SR) is a challenging task in machine learning that involves finding a mathematical expression for a function based on its values. Recent advancements in SR have demonstrated the effectiveness of pre-trained transformer-based models in generating equations as sequences, leveraging large-scale pre-training on synthetic datasets and offering notable advantages in terms of inference time over classical Genetic Programming (GP) methods. However, these models primarily rely on supervised pre-training goals borrowed from text generation and overlook equation discovery objectives like accuracy and complexity. To address this, we propose TPSR, a Transformer-based Planning strategy for Symbolic Regression that incorporates Monte Carlo Tree Search into the transformer decoding process. Unlike conventional decoding strategies, TPSR enables the integration of non-differentiable feedback, such as fitting accuracy and complexity, as external sources of knowledge into the transformer-based equation generation process. Extensive experiments on various datasets show that our approach outperforms state-of-the-art methods, enhancing the model's fitting-complexity trade-off, extrapolation abilities, and robustness to noise.

==> NeurIPS2023/table_figs_tex/pairgrid_blackbox.tex <==
\begin{figure}[!ht]
% \centering
\includegraphics[width=0.95\linewidth]{ArXiv/figures/median_pairgrid-pointplot_r2_test_model_size.pdf}
% \captionsetup{font=footnotesize}
\caption{Performance comparison of \modelname and SRBench algorithms in terms of Accuracy-Complexity-Time on \textit{Black-box} dataset. Algorithms are sorted based on median $R^2$ score on test set. TPSR ($\lambda=0, 0.1$) achieves the best fitting performance while having a controllable complexity and lower inference time compared to the GP-based SR algorithms. The error bars represent the 95\% confidence interval and "$*$" refers to SR methods.
}
\label{fig:blackbox_parigrid}
\end{figure}

==> NeurIPS2023/table_figs_tex/tableCache.tex <==

\begin{table}[htbp]
\centering
\caption{Average computation time (sec.) of \modelname on 119 equations of Feynman dataset. The results are for $\lambda=0.1$.}
\begin{tabular}{ccc}
\toprule
Sequence Cache & Top-K Cache & Time (sec.) \\
\midrule
\xmark  & \xmark & 318.43 \\
\xmark  & \cmark & 270.91 \\
\cmark  & \xmark & 236.05 \\
\cmark  & \cmark &  137.15 \\
\bottomrule
\end{tabular}
\label{table-PMLB}
\end{table}

==> NeurIPS2023/table_figs_tex/tableInDomain.tex <==
\begin{table}[t]
\caption{Performance of \modelname compared with beam search and sampling decoding strategies on the in-domain synthetic data of \cite{Kamienny-E2E-symbolic-NIPS-2022}}
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
Model              & $\uparrow$ $R^2>0.99$ & $\uparrow$ $R^2$ & $\uparrow$ $\mathrm{Acc}_{0.1}$ & $\uparrow$ $\mathrm{Acc}_{0.01}$ & $\uparrow$ $\mathrm{Acc}_{0.001}$ & $\downarrow$ $Complexity$ \\
\midrule

E2E+Beam & 0.657 &0.782 & 0.461 & 0.298  &  0.2 & 38.37 \\
E2E+Sampling & 0.640 & 0.794 &  0.472 & 0.332 & 0.208 & 39.82\\
\midrule
TPSR (\textcolor{red}{$\lambda$=0}) & 0.702 &0.828 &\textbf{0.550}& \textbf{0.416} &\textbf{0.333}&67.11\\
TPSR (\textcolor{red}{$\lambda$=0.1})  &\textbf{0.708}&\textbf{0.833}&0.514&0.326&0.213&40.31\\
TPSR (\textcolor{red}{$\lambda$=0.5})  &0.697&0.830&0.459&0.274&0.184&36.55\\
TPSR (\textcolor{red}{$\lambda$=1}) &0.691&0.827&0.439&0.271&0.176&\textbf{35.67}\\
\arrayrulecolor{black}\bottomrule
\arrayrulecolor{black}\bottomrule
\end{tabular}
}
\label{table-indomain}
\end{table}

